How Far Are Large Multimodal Models from Human-Level Spatial Action? A Benchmark for Goal-Oriented Embodied Navigation in Urban Airspace

Large multimodal models (LMMs) show strong visual-linguistic reasoning but their capacity for spatial decision-making and action remains unclear. In this work, we investigate whether LMMs can achieve embodied spatial action like human through a challenging scenario: goal-oriented navigation in urban 3D spaces. We first spend over 500 hours constructing a dataset comprising 5,037 high-quality goal-oriented navigation samples, with an emphasis on 3D vertical actions and rich urban semantic information. Then, we comprehensively assess 17 representative models, including non-reasoning LMMs, reasoning LMMs, agent-based methods, and vision-language-action models. Experiments show that current LMMs exhibit emerging action capabilities, yet remain far from human-level performance. Furthermore, we reveal an intriguing phenomenon: navigation errors do not accumulate linearly but instead diverge rapidly from the destination after a critical decision bifurcation. The limitations of LMMs are investigated by analyzing their behavior at these critical decision bifurcations. Finally, we experimentally explore four promising directions for improvement: geometric perception, cross-view understanding, spatial imagination, and long-term memory. The project is available at: https://github.com/serenditipy-AC/Embodied-Navigation-Bench.

==> 3.method.tex <==

\section{Methodology}
%To address the mentioned above challenges, we propose an embodied agent named DeliverGPT, presented in Fig. \ref{framework}.
%%VLMs possess vision-language understanding capability, while LLMs have commonsense reasoning ability. However, they lack spatial understanding and reasoning in the real 3D world, which makes it challenging to generate effective and robust low-level drone actions directly. To close this gap, 
%We first construct agent's comprehensive perception of the environment (Section \ref{perception}). We then develop spatial planning capabilities for the agent (Section \ref{planning}) and convert the planning results into drone motion (Section \ref{motion}).
%%we first obtain an LLM-understandable environment representation called the semantic graph in the perception module. Subsequently, the LLM can perform planning on the semantic graph, determining which node to navigate to next and addressing the "where to" question. The motion module then utilizes a deterministic policy for low-level action control, addressing the "how to go" question. 
%Additionally, we design the memory module to assist the agent in spatial perception and planning for similar delivery tasks (Section \ref{memory}). 

% We first develop three foundational mechanisms of the embodied agent's spatial cognition: size constancy, viewpoint invariance, and spatial perspective-taking. These enable EmbodiedNav to establish spatial awareness relying solely on RGB observations and memory. Subsequently, these abilities are integrated into the agent's design to facilitate the mapping from perception to action.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/planning_process.pdf}
  % \vspace{-0.2cm}
	\caption{Overview of the proposed aerial agent for goal-oriented navigation. Our agent consists of six modules: Localization, Planning, Imagination, Decision-Making, Active Perception, and Memory.}
	\label{fig:framework}
 % \vspace{-0.4cm}
\end{figure*}

The proposed agent consists of six modules, as shown in Figure \ref{fig:framework}. 
The \textbf{localization} module determines changes in the spatial relationships between the agent and key objects in the environment based on historical and current observations, as well as the sequence of actions. The \textbf{planning} module provides the latest plan and tracks current progress. The \textbf{imagination} module utilizes spatial reasoning to predict the changes in position and observations resulting from the execution of each action. The \textbf{decision-making} module selects the action that best aligns with the current plan and maximizes the likelihood of observing or locating the target, based on the outcomes of the counterfactual reasoning. If the agent is uncertain about which action to take, it can engage in \textbf{active perception} to gather additional sensory information before making a revised decision. Throughout this process, the RGB observation and output of each module are updated in the \textbf{memory} module, providing information to other modules.


% The \textbf{localization} module outputs the latest plan and current progress. The \textbf{perception-driven action generation} module converts steps in the plan into an iterative algorithm, which outputs the agent's actions. 
%\subsubsection{Perception} \label{perception}
%
%Spatial perception forms the foundation of planning, particularly in large-scale urban environments where semantic information is sparse, which requires integrating historical observations and extracting spatial semantic information. 
%To address this, we develop a semantic graph to facilitate this process, composed of a textual conceptual level $C_t$ and a metric level $M_t$. The conceptual level facilitates understanding and reasoning for the LLM, while the metric level facilitates navigation for the UAV. 
%%Based on a comprehensive understanding of urban architectural structure and object detection, this module actively constructs and expands a 3D scene graph to represent the explored urban environment. 
%The conceptual level of the 3D Semantic Graph Generation is a layered graph that encompasses spatial concepts (nodes, denoted as ${N_{j,t}}$) at multiple levels of abstraction, along with their corresponding relationships (edges, denoted as $E_{k,t}$). 
%The edges of the graph illuminate the topological relationships among semantic concepts across various nodes.
%This representation has recently emerged as a notable high-level abstraction for capturing 3D urban buildings or scenes using drones. %In this context, we delineate three distinct levels within the 3D scene graph: scene, floors, and objects. 
%
%
%The generation and iterative process of the semantic graph are as follows. 
%Suppose the observation $o_t$ at time $t$ consists of RGB $v_t$, Depth $d_t$, and pose $m_t$. VLM possesses the vision-language understanding capability for a single image. Employing a prompt of scene understanding $P_{scene}$ (Figure \ref{prompt}a), the VLM can describe the building elements in the RGB image in textual form $b_t$:
%\begin{equation}
%	{b_t} = {\rm{VLM}}({v_t}, {P_{scene}})
%\end{equation}
%Then the conceptual level of semantic graph ${C_t} = \{ ({N_{j,t}},{E_{k,t}})\} $ is derived by:
%\begin{equation}
%	{C_t} = {\rm{LLM}}({b_t},{C_{t - 1}},{P_{graph}})
%\end{equation}
%where the LLM is continuously employed to update the graph taking the image description ${b_t}$, previous conceptual part ${C_{t - 1}}$, and graph generation prompt ${P_{graph}}$ (Figure \ref{prompt}b) as input. 
%%RGBD images serve as input to the LLM, enabling the determination of whether the elements within the current building semantic graph are within the current visual field, and whether additional objects are present within the field of view. The information obtained from target recognition is then integrated into the graph. By utilizing RGBD images and semantic segmentation images, the depth of each segmented object can be derived. Consequently, by combining this depth information with the agent's pose, the 3D coordinates of each perceived object can be estimated.
%For the metric level, we obtain it through the SLAM algorithm, which leverages depth and pose sensors carried by the UAV to perceive surrounding structures, roads, and other environmental features. By continuously observing the environment and estimating the robot's position, SLAM algorithms can simultaneously construct an accurate map (Appendix \ref{slam_app}).
%\begin{equation}
%	{M_t} = {\rm{SLAM}}({d_t},{m_t})
%\end{equation}
%
%Additionally, the building semantic graph can be initially established by leveraging prior knowledge of urban architectural structure. For instance, it is well-established that a building's main entrance is typically situated on the ground floor, while the rooftop often features an apron. 
%%Similarly, parks commonly have entrances facing the roadside, with bridges positioned over rivers. We have compiled semantic graphs for prevalent building types encountered within the city, encompassing office buildings, houses, commercial and residential structures, commercial districts, and parks. 
%%As the drone ascends above a specific urban scene, if a delivery has been previously made in this scene, the conceptual level of the semantic graph formed in memory will serve as the initial value $S_0$. Otherwise, the scene is assessed to determine its corresponding type, and the rough conceptual level of the semantic graph for that type is used as the initial value.

\subsection{Localization} \label{localization}

Since the goal is given at the starting position, it is necessary to determine what motion the current agent has done relative to the starting position. This is crucial for subsequent planning.
We can derive the localization information ${A_{loc,t}}$ via the multimodal understanding capability of LMM:
\begin{equation}
    {A_{loc,t}} = {\rm{LMM}}(\{ {o_i}\} _{i = 0}^t,\{ {a_j}\} _{j = 0}^t|Q_{loc}),
\end{equation}
where $Q$ is the localization prompt.

\subsection{Planning} \label{planning}

% \begin{figure*}[!t]
% 	\centering
% 	\includegraphics[width=5.5in]{figures/planning_process.pdf}
% 	\caption{The design of embodied CoT for the Track$^2$ Task Decomposition module, mainly including plan evaluation, perception inference, and route inference. The perception inference and route inference stages are specifically designed based on spatial imagination and spatial association, respectively. The resulting plan is better equipped to handle goal-oriented navigation tasks in urban spaces.}
% 	\label{planning_module}
%     \vspace{-0.5cm}
% \end{figure*}

The purpose of this module is to generate a high-level plan for gradually approaching the goal location. Plans produced directly by LMMs are often vague, random, and difficult to integrate with the subsequent action generation module. Moreover, such plans typically focus solely on the agent's movement, neglecting interdependency between perception and route. To navigate towards the target location, we need a good perspective and more clues to support planning. In urban environments, being too far from or too close to surrounding buildings can affect observation. 
%We have designed an embodied CoT that incorporates imagination and associative abilities from spatial cognition, considering both perception and route in task decomposition.

LMM is prompted to perform common-sense reasoning to infer the relationship between the final goal location and the current scene, even without complete environmental knowledge. For instance, a "large billboard" might be on the middle floors of an office building, while a "helipad" should be on the rooftop. Subsequently, a complete chained \textbf{perception} plan is provided, progressively narrowing the perception and search area, such as focusing from the entire building down to the vicinity of the elevators, as shown in the diagram.

Upon obtaining the perception plan, we need to infer a specific \textbf{route} that aligns the agent’s field of view with the perception plan. We further standardize route generation, including the start, flight, and end points. Additionally, we activate the agent's spatial associative ability to help select the route's start and end points. For example, as illustrated, the building entrance is likely facing the road, so starting the search from the roadside of the building may be a good choice. By concatenating the above step-by-step reasoning process, we can derive the final track plan and progress status. This track$^2$ task composition adapts to the perceptual challenges posed by open-ended urban environments:
\begin{equation}
    {A_{plan,t}} = {\rm{LMM}}({A_{loc,t}},{o_t}|Q_{plan})
\end{equation}
where $Q_{plan}$ is the planning prompt.

% The role of the spatial planning module is to output a high-level plan to approach the goal location gradually, as shown in Figure \ref{planning_module}. It begins by retrieving historical sequences of RGB observations and plans from the memory module. The self-reflection module then determines whether the plan needs adjustment. If no adjustment is needed, it evaluates whether the current step in the plan is complete. If complete, it outputs the next step; otherwise, it continues with the current step.

% If the plan requires creation or modification, spatial imagination is activated. Imagination is needed because the goal-location is not directly observable; the agent must imagine its spatial relationship with the currently observed urban elements. The focus is on the relationship between the goal and the scene, which consists of abstract spatial regions not easily identifiable in the view. An imagination generator is used to create visualizations of common spatial relationships between the goal and buildings, enhancing LMM's reasoning. Through images and prompts, the agent gains spatial perspective-taking, allowing it to understand that buildings have multiple sides in 3D space. To find the final goal, the agent must move around obstructions and approach the goal's vicinity, observing from a specific camera pan angle. This imagination narrows the search area, enabling quick goal localization. Additionally, the agent considers the relationship between easily identifiable urban elements or objects and the goal, such as a main entrance facing a road, which aids in determining the search direction and speeding up navigation.

% Using the results of this imagination, navigation is broken down into feasible steps. The plan is stereoscopic, involving vertical and horizontal movements and camera angle adjustments for effective perception. The final output is the updated plan and the current step to execute.

%Spatial planning capability refers to the agent's ability to determine ``where to go" in a three-dimensional open world. Through dynamic perception and a series of decisions, the agent gradually approaches the goal location. We combine the conceptual level of the semantic graph with the commonsense reasoning ability of LLM to construct this capability.
%
%%Spatial planning can be divided into two steps: next node selection and mapping. Leveraging the semantic graph constructed earlier, we can utilize the commonsense reasoning abilities of the Language Models with Memory (LLMs) to achieve planning. 
%
%We emphasize that instead of directly generating drone actions, this module focuses on high-level planning: determining which node within the conceptual level of the semantic graph to navigate to next. This effectively harnesses the commonsense reasoning capabilities of LLM while mitigating its limitations in embodied capabilities. The layered structure of the conceptual level can be easily converted into textual form and understood by the LLM. The thought process behind the prompt for planning is as follows: first, clarifying the current node where the agent is located and emphasizing the target to be found; second, finding a node in the next layer of the current node, which either belongs to the final target location or is close in proximity to the final location, as shown in Figure \ref{prompt}(c) in Appendix. This effectively leverages the commonsense reasoning ability of LLM to its full potential. For instance, when the drone needs to navigate to ``underneath the red tree next to the building'', even if the red tree is not yet observed in its field of view, LLM can still infer the next step to proceed towards the node ``ground floors'' based on the reasoning that ``trees are mostly found on ground floors.''
%\begin{equation}
%	N_{i,t}^{{\rm{goal}}} = {\rm{LLM}}({C_t},{P_{plan}})
%\end{equation}

%%%每个小节有个小结论和总结

\subsection{Imagination}
The Imagination module utilizes spatial reasoning to predict the changes in position and observations resulting from the execution of each action. If the prompt is denoted as $Q_{imgn}$, the prediction outcome $A_{k,t}$ of each potential action $k=1,2,...,10$ can be calculated as:
\begin{equation}
    {A_{k,t}} = {\rm{LMM}}({A_{plan,t}},{A_{loc,t}},{o_t}|{Q_{imgn}}).
\end{equation}

\subsection{Decision-Making}
The Decision-Making module selects the action that best aligns with the current plan and maximizes the likelihood of observing or locating the target. This selection is based on counterfactual reasoning performed by the LMM with prompt $Q_{DM}$:
\begin{equation}
    k = {\rm{LMM}}(\{ {A_{k,t}}\} _{k = 1}^{10},{A_{plan,t}}|{Q_{DM}})
\end{equation}
If LMM is confident to the decision, then \(k \to {a_t}\)

\subsection{Active Perception}

The Active Perception module is triggered when the agent is uncertain about which action to take. It gathers additional observation information $o_{add,t}$ by exploring the environment before making a revised decision. Here, we allow the aerial agent to obtain views in the front, left, back, right, up, and down directions respectively. Input it back into LMM so that it can comprehensively determine which action should be taken:
\begin{equation}
    \hat k = {\rm{LMM}}({A_{plan,t}},{A_{loc,t}},{o_{add,t}}|{Q_{imgn}},{Q_{DM}})
\end{equation}

Finally, we derive \(\hat k \to {a_t}\).




% \subsection{Perception-Driven Action Generation} \label{motion}

% We build this module to further decompose each step of the aforementioned track$^2$ plan into a combination of low-level control actions. We employ a more anthropomorphic hardware setup, executing actions based solely on continuous RGB observations, without relying on depth sensors or GPS data. In practice, humans similarly depend on changes in objects and scenes within their field of view to assess relative distances, directions, and the three-dimensional characteristics of urban objects. This involves micro-level, pose-level spatial cognition mechanisms. Specifically, humans can determine relative distances through the size of objects and their changes, known as \textbf{size constancy}. By matching continuous visual features, we recognize the same three-dimensional object from different viewpoints, referred to as \textbf{viewpoint invariance}. Moreover, humans can understand three-dimensional objects through perspective elements like edges of urban objects, referred to as \textbf{spatial perspective-taking}. Details can be found in Appendix \ref{sec::appendix::spatial_cog}. 

% Therefore, action generation can be driven by visual perception: inputting RGB observations into the LMM to obtain fundamental visual semantic features, from which our defined spatial cognition-aware deterministic policy can infer relative spatial relationships and subsequently determine actions. We primarily utilize the object recognition and rough localization capabilities of the LMM. Although the LMM cannot provide precise visual localization, its open-vocabulary visual question-answering capability is well-suited for urban navigation scenarios. This is because the visual targets we inquire about are likely to be part of buildings or other urban elements, such as "three floors up from the ground." Suppose the spatial cognition-aware deterministic policy is $\Gamma$ and a step in the track$^2$ plan is  $S = \left[ {{c_1},{c_2};{r_1},{r_2},{r_3}} \right]$, where ${c_1},{c_2}$ are perception track content and ${r_1},{r_2},{r_3}$ belong to route track. We can derive:
% \begin{equation}
%     {V_c},\Phi ,{\rm P} = \Gamma \left( S \right)
% \end{equation}
% where ${V_c}$ represents the semantic perception state of $S$ upon completion. $\Phi$ is the mapping function from semantic perception states to actions. ${\rm P}$ denotes the promotor for question answering concerning the semantic perception features that need to be extracted. 
% Agent's actions are generated via Algorithm \ref{action_gen_alg}. 

% Figure \ref{skill_module} provides an example: the perception area is the entire side of the building, flying around along the building's edge. This primarily utilizes the rough image localization function of LMM. Different situations of the building in the field of view correspond to different relative positional relationships, from which the necessary actions can be deduced. We also provide additional examples to illustrate our proposed deterministic policy and iterative algorithm, such as moving to an abstract spatial location relative to the scene/building ($move\_to()$), adjusting the view ($adj\_view()$), and approaching an object/element in view ($approach()$). See the Appendix \ref{sec::appendix::action_gen} for details.


% \begin{algorithm}[!t] 
% \caption{Perception-Driven Action Generation}
% {\bf Input:} %算法的输入， \hspace*{0.02in}用来控制位置，同时利用 \\ 进行换行
% $S,{V_c},\Phi ,{\rm P}$, ${\rm{LMM}} $, $o_t, {{\alpha _t}}$ \\
% {\bf Output:}  ${a_t}$ %算法的结果输出
% \begin{algorithmic}[1]
%     \REPEAT
%         \STATE ${V_{{\rm{LMM}}}} = {\rm{LMM}}\left( {{o_t},{\rm P}\left( {{c_1},{c_2}} \right)} \right)$
%         \IF{${V_{{\rm{LMM}}}} =  = {V_c}$}
%             \STATE \textbf{break}
%         \ELSE
%             \STATE ${a_t} = \Phi \left( {{V_{{\rm{LMM}}}},{\alpha _t}} \right)$
%         \ENDIF
%     \UNTIL Reach maximum iteration limit 
% \end{algorithmic}
% \label{action_gen_alg}
% \end{algorithm}

%After determining the next node to navigate to, we need to address how the drone moves. This process can be divided into three steps: grounding, mapping, and action generation. Grounding involves approximating the position of the selected node within our RGB observation. Subsequently, by incorporating depth and pose information, we obtain the coordinate point $({x_t},{y_t},{z_t})$ of that position on the metric level in the semantic graph. 
%\begin{equation}
%	N_{i,t}^{{\rm{goal}}} \to ({x_t},{y_t},{z_t}) \sim {M_t}
%\end{equation}
%After deriving the exact coordinate on the metric level of semantic map, the delivery agent is equipped with a deterministic policy $G\left(  \cdot  \right)$
%to help it navigate to the goal. The full motion algorithm is in Appendix \ref{grounding}.
%\begin{equation}
%	{a_t} = G\left( {({x_t},{y_t},{z_t}),{M_t}} \right)
%\end{equation}

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=\linewidth]{figures/skill.pdf}
% 	\caption{Perception-driven action generation: example of flying around an area of interest while maintaining a relatively constant distance and ensuring effective camera perception. To accommodate the LMM, the field of view is divided into a grid to determine the rough location of the area of interest. }
%  \vspace{-0.5cm}
% 	\label{skill_module}
% \end{figure}

%At $t=0$, the building fully appears in view, indicating the agent is at an appropriate distance from the area of interest, resulting in a move-right action. At $t=1$, the building appears to the agent's front left; to re-center the building in view, the agent outputs turn-left and move-right actions. At $t=2$, the building occupies a smaller area in the view, suggesting increased distance, which can impair the agent's perception, resulting in a move-forward command. The $t=3$ RGB observation confirms the view adjustment goal is achieved. Throughout different viewpoints during the flight, the ability to consistently recognize the building of interest showcases the viewpoint invariance ability. Inferring distance based on the perceived area of the building in view illustrates the size constancy ability.

% To facilitate mapping steps in the plan to actions, we extract common steps into skills, including: moving to an abstract spatial location relative to the scene/building ($move\_to()$), flying around a target ($fly\_around()$), adjusting the view ($adj\_view()$), and approaching an object/element in view ($approach()$). These skills also provide feasibility constraints for step decomposition in planning. The skills are grounded in spatial cognition principles, enabling spatial awareness such as relative distance and scene-object consistency, thereby establishing action mapping, as shown in Figure \ref{skill_module}.







\subsection{Memory} \label{memory}
% As previously mentioned, the capabilities of spatial cognition and viewpoint invariance are derived from the comparison and synthesis of continuous RGB observations. 
% The agent, built upon foundational LMM capabilities and spatial cognition, relies on memory for its planning, skill, and action execution modules. 
The memory is organized into three categories: RGB observations, plan history, and action history at each time moment. Each module retrieves the necessary components from memory as inputs as needed. Suppose the memory module is $\mathcal{M}_t$, the update content is:
\begin{equation}
    {{\cal M}_t} = {{\cal M}_{t - 1}} \cup \{ {o_t},{A_{plan,t}},{a_t}\} .
\end{equation}

% At any given time $ t $, the track$^2$ task decomposition module retrieves historical RGB observations, previous plans, and plan progress from the memory. During the plan evaluation phase, the system evaluates whether the plan from time $ t-1$ requires adjustments or if the execution has reached a particular step. If modifications are made or steps are updated, the new plan or step is stored in the memory for time $ t $. If no updates occur, the plan and step from $ t-1 $ are stored for time $ t $. To manage the potential overflow of RGB observations beyond the token limit of the LMM, retrieval is done through uniform sampling, ensuring that observations from times $ 0 $ and $ t-1 $ are retained in the sequence.

% The perception-driven action generation module retrieves RGB observations and actions from the start of the current step to the latest moment. From time $ t-n $ to $t$, it uses the latest plan and the required step to execute the corresponding skill. All relevant RGB observations and actions from this interval are retrieved. Historical RGB observations are critical for maintaining size constancy and viewpoint invariance—helping to judge distances and determine the orientation of areas of interest through visual feature matching. Historical actions facilitate understanding changes in the field of view and, in cases of rapid viewpoint shifts causing target loss, allow for reasoning about the agent's relative position through action backtracking. The skill executed and actions taken at time $ t $ are then stored in memory for that time.

% Memory enables individuals to remember paths, directions, or waypoints required to reach a destination, helping in both habitual and novel navigation tasks.

%\textbf{Short-term memory: }
%For each navigation, in addition to the semantic graph, historical decisions generated by the LLM are recorded to facilitate the next reasoning step.
%
%\textbf{Long-term memory: }
%Equipped with a memory of historical deliveries, the agent acquires knowledge of the environment surrounding the delivery location and gains experience in spatial planning. Leveraging this prior experience enables agent to execute tasks with greater efficiency, mirroring the enhancement of human skills through repetitive practice.
%We have devised a distributed memory mechanism within urban spaces that facilitates the storage and retrieval of acquired knowledge, as shown in Fig. \ref{Fig_4}. This encompasses the construction of semantic maps and the documentation of historical delivery trajectories. Contrary to reinforcement learning-based models, which encapsulate knowledge within model parameters, our approach renders the delivery knowledge explicit, logical, and more closely resonant with human cognitive processes. Upon the drone's approach to the delivery location, the relevant memory pertaining to that location is activated. This obviates the need to reconstruct the semantic graph from scratch based on current observations with each delivery attempt. Instead, the pre-remembered semantic graph serves as a more comprehensive and precise initial condition, derived from multiple delivery iterations. 
%This not only provides the agent with a fundamental comprehension of the delivery environment but also enhances the efficiency and accuracy of the delivery process. Moreover, when tasked with delivering to a novel destination, the agent may initially necessitate multiple exploratory attempts to ascertain the precise location. However, upon subsequent deliveries, leveraging accrued experience, the agent is able to expedite the process by navigating directly to the delivery site via an optimized sequence of nodes. 


%Upon each delivery's completion, the experienced node list is stored. Optimal strategies are identified by summarizing essential nodes from various plans, employing LLMs. For instance, a recorded trajectory included the node sequence: ground floors - yellow tree - door - middle floors - billboard - ground floors - ground. The deduced optimal sequence for this trajectory was established as: middle floors - billboard - ground floors - ground. This memory mechanism significantly augments the efficiency of delivery across a broad spectrum of similar tasks. As this process repeats, the Language Model-based Planner's efficiency significantly improves. 







%\subsection{Vision-Language Navigation}
%Navigator 1 is designed for vertical navigation of UAVs. Given the complexity of vertical dimensions in urban environments, we employ a combination of common sense reasoning from a large-scale model, visual observations, and the building semantic graph to determine the target point's corresponding floor level. Navigator 1 utilizes a rule-based approach to initially estimate the approximate height of the building and subsequently identify the height range of the target floor, enabling navigation to the desired altitude.
%
%Navigator 2, on the other hand, focuses on horizontal search and navigation of UAVs. Following a rule-based configuration, the UAV flies around the target building while maintaining the camera's alignment with the building. In this process, RGBD images are fed into the large-scale model to determine the presence of the target object. If the object is not detected, the UAV continues flying until the target object is found. Additionally, leveraging the multimodal capabilities of the large-scale model, multiple iterations of fuzzy localization are performed to approach the vicinity of the final target destination.
%
%\begin{figure*}[!t]
%	\centering
%	\includegraphics[width=5.5in]{figures/Fig 3/Fig 3.jpg}
%	\caption{In Navigator 2, when the large model determines the presence of the target object being searched for in the image, the current perspective is divided into nine sub-images. The large model further identifies the sub-image in which the object is located, enabling rough grounding. By incorporating depth imaging to estimate its distance, multiple iterations are performed to eventually reach the vicinity of the target object.}
%	\label{Fig_3}
%\end{figure*}

